Precise Asymptotic Generalization for Multiclass Classification with Overparameterized Linear Models

We study the asymptotic generalization of an overparameterized linear model for multiclass classification under the Gaussian covariates bi-level model introduced in Subramanian et al.~'22, where the number of data points, features, and classes all grow together. We fully resolve the conjecture posed in Subramanian et al.~'22, matching the predicted regimes for generalization. Furthermore, our new lower bounds are akin to an information-theoretic strong converse: they establish that the misclassification rate goes to 0 or 1 asymptotically. One surprising consequence of our tight results is that the min-norm interpolating classifier can be asymptotically suboptimal relative to noninterpolating classifiers in the regime where the min-norm interpolating regressor is known to be optimal. The key to our tight analysis is a new variant of the Hanson-Wright inequality which is broadly useful for multiclass problems with sparse labels. As an application, we show that the same type of analysis can be used to analyze the related multilabel classification problem under the same bi-level ensemble.

==> app_I_technical_lemmas.tex <==
\section{Miscellaneous lemmas}\label{sec:technical-lemmas}
\begin{lemma}[Coupling of quadratic forms]\label{lemma:psd-coupling}
Let $\mB \in \RR^{n \times m}$ be an arbitrary real matrix and $\mM \in \RR^{n \times n}$ be a PSD matrix. Then for any vector $\vx \in \RR^m$, we have 
\begin{equation}
    \lambda_n(\mM) \vx^\top \mB^\top \mB \vx \le \vx^\top \mB^\top \mM \mB \vx \le \lambda_1(\mM) \vx^\top \mB^\top \mB \vx. \label{eq:psd-coupling}
\end{equation}
\end{lemma}
\begin{proof}
For any PSD matrix $\mC$, the matrix $\mB^\top \mC \mB$ is PSD. 
In particular, $\mC$ has a unique square root $\mC^{1/2} \in \RR^{n \times n}$ with $\mC^{1/2} \mC^{1/2} = (\mC^{1/2})^\top \mC^{1/2} = \mC$. We thus have
\begin{align}
    \vx^\top \mB^\top \mC \mB \vx &= \vx^\top \mB^\top \mC^{1/2} \mC^{1/2} \mB \vx \\
    &= \norm{\mC^{1/2} \mB \vx}_2^2 \ge 0. \label{eq:psd-form}
\end{align}

Hence 
\begin{align}
    \lambda_1(\mM)  \vx^\top \mB^\top \mB \vx - \vx^\top \mB^\top \mM \mB \vx = \vx^\top \mB^\top (\lambda_1(\mM)\mI_n - \mM) \mB \vx. 
\end{align}
Since $\mM \preceq \lambda_1(\mM) \mI_n$ by definition, $\lambda_1(\mM)\mI_n - \mM$ is a PSD matrix. Hence by applying \cref{eq:psd-form}, we conclude that 
\begin{align}
    \lambda_1(\mM)  \vx^\top \mB^\top \mB \vx - \vx^\top \mB^\top \mM \mB \vx \ge 0,\label{eq:psd-upper-bound}
\end{align}
which gives the upper bound in \cref{eq:psd-coupling}.

Similarly, $\mM \succeq \lambda_n(\mM) \mI_n$, so an analogous argument 
\begin{align}
    \lambda_n(\mM)  \vx^\top \mB^\top \mB \vx - \vx^\top \mB^\top \mM \mB \vx \le 0,\label{eq:psd-lower-bound}
\end{align}
which gives the lower bound in \cref{eq:psd-coupling}. 
\end{proof}


Next, we prove the elementary anti-concentration result that we will need.
\begin{proposition}[Gaussian anticoncentration]\label{prop:gaussian-anticoncentration}
Let $\vx \sim N(0,\mathbf{I}_d)$ be a standard Gaussian vector, and let $\vv \in \RR^d$ be arbitrary deterministic vector. Then 
\[
\Pr[\abs{\ev{\vx, \vv}} \le \epsilon] \le \frac{2\epsilon}{\sqrt{2\pi}\norm{v}_2}.
\]
\end{proposition}
\begin{proof}
Note that $\ev{\vx, \vv}$ is a linear projection of a standard multivariate Gaussian, so it is itself a one-dimensional Gaussian. It is also clearly zero mean, and its variance is just give by the squared norm of $\vv$. So $\ev{\vx, \vv} \sim N(0, \norm{\vv}_2^2)$. Now we have 
\[
\Pr[\abs{\ev{\vx, \vv}} \le \epsilon] = \frac{1}{\sqrt{2\pi}\norm{\vv}_2}\int_{-\epsilon}^{\epsilon} \exp(-\frac{x^2}{\norm{\vv}_2^2})dx \le \frac{2\epsilon}{\sqrt{2\pi}\norm{\vv}_2}.
\]
\end{proof}


